Cosmic Visions Dark Energy: Science

Cosmic surveys provide crucial information about high energy physics including strong evidence for dark energy, dark matter, and inflation. Ongoing and upcoming surveys will start to identify the underlying physics of these new phenomena, including tight constraints on the equation of state of dark energy, the viability of modified gravity, the existence of extra light species, the masses of the neutrinos, and the potential of the field that drove inflation. Even after the Stage IV experiments, DESI and LSST, complete their surveys, there will still be much information left in the sky. This additional information will enable us to understand the physics underlying the dark universe at an even deeper level and, in case Stage IV surveys find hints for physics beyond the current Standard Model of Cosmology, to revolutionize our current view of the universe. There are many ideas for how best to supplement and aid DESI and LSST in order to access some of this remaining information and how surveys beyond Stage IV can fully exploit this regime. These ideas flow to potential projects that could start construction in the 2020's.

==> boa.tex <==
%\subsubsection{Massively multiplexed spectroscopy for Cosmology}

By the mid 2020s, DESI will have completed its 5-year survey of the northern hemisphere and LSST will be operating in the south. DESI is expected to obtain redshifts of around 24 million galaxies. LSST will have many more objects in its catalog, some four billion, but it scientific reach will likely be limited by the lack of redshifts for those objects. In fact, it is likely that LSST will not be dominated by statistical precision, but instead by the unavoidable systematics associated with photometric redshift errors. However, at the same time LSST will be the ultimate targeting survey, being deeper and more accurate than anything else available at the time. Therefore, one alluring possibility is that the next generation large scale structure experiment will be a spectroscopic experiment obtaining spectra for hundreds of millions of LSST-detected targets. 

Which and how many LSST objects should be targeted should be dictated by the scientific case that develops over the next decade. Going to higher redshift means obtaining fewer spectra, but this cost might be outweighed by the fact that more volume is probed and the structure is less nonlinear and therefore easier to compare with theory.   Taking more spectra might become more compelling if theoretical advances in understanding the non-linear clustering of multiple populations of sources covering the same area continue at the same rate. We argue that DOE should continue R\&D into theoretical understanding of non-linear LSS in order to extract maximum information using multiple-tracer methods and possible testing of gravity through non-canonical observables. 
%In order to be interesting, this experiment would need to be at least an order of magnitude more ambitious that DESI: a factor o a few does not cut it since combination catalogs combining all available redshift surveys will reach around 100 million sources (according to Chris's counting). 
%One ambitious possibility is to increase the number of spectra by an order of magnitude, obtaining several hundred million spectra of LSST galaxies. There are two main ways of doing this: either by going after more objects (a few hundred millions over the existing survey footprints) or by going after more volume (fainter objects at higher redshfit). 

%An argument for more volume is that linear theory is more applicable at higher redshift so comparing theory to the observations might be less complex. %is something that we know how to do. But 
%Moreover, a deep $g$-band flux limited survey might also be interesting for astronomy in general and might allow for a new multi-agency experiment following the model established by LSST. How might a billion object $g$-band limited experiment look like?

\subsubsection{Spectrograph}

The DESI spectrogram will take spectra of 5000 objects using 10 spectrographs with 500 traces each. The PFS instrument is similar and Maua Kea Spectroscopic explorer is somewhat more ambitious. Assuming a modest improvement in technology to a 2000 trace-spectrograph taking tens of thousands each, it seems that ten of thousands traces simultaneously should be technologically feasible. An important improvement would be to extend the redshift range into the red using new Ge CCDs. The spectral resolution requirement should be studied more carefully but likely the current sweet-spot of around $R\sim2000$ should continue be sufficient.

\subsubsection{Redshifting sources}

There are two different categories of redshift classifications:  i) optical identification of OII; examples include zcosmos, VVDS and VIPERS; ii) classification through Lyman-$\alpha$ emission and UV interstellar absorption features.

\subsubsection{Fiber system}
It is unlikely that the DESI model with robotic fiber positioners will scale to such task. Making mechanical positioners smaller is difficult: a solid state solution would be preferable. There are several options available, all of which would require further R\&D. One possibility is to route light around using image slicer and/or micromirrors arrays. A second possibility is to project light from large sky area into a single fiber using lenslet arrays, but this will likely have problems with phase-space conservation. Perhaps the most compelling strategy would be to project thousands of fibers along the same spectroscopic trace and only let the light pass through selected fibers using microshutters or an equivalent strategy. This would allow one to fill the focal plane with fibers at packing efficiency around 50\% and then use dithering algorithms to account for dead space.

\subsubsection{IGM intensity mapping}
As the number density of fibers increases, there will inevitably be fiber positioning inefficiencies in any system with a finite spectral trace "patrol radius" (including current DESI and PSF designs). However, large number of fibers that are not taking object spectra could be used for Lyman-$\alpha$ (and other line) intensity mapping of the IGM. Moreover, even for spectra with objects on them, since the noise is dominated by the sky noise, their statistical utility after the model for the targeted object is subtracted should be roughly the same (but there might be subtle systematic effects associated with this procedure). DOE should investigate the scientific reach of this technique.





==> mgscience.tex <==
\newcommand{\sfig}[2]{
\centering
%\begin{center}
\includegraphics[width=#2]{#1}
%\end{center}        
}
\newcommand{\Sfig}[2]{
%\begin{center}
    \begin{figure}[htbp]
    \sfig{#1.pdf}{0.55\columnwidth}
   %  \end{center}
   \caption{#2} %{\small #2}}
    \label{fig:#1}
    \end{figure}
}
\newcommand{\Sfigtwo}[3]{
%\begin{center}
    \begin{figure}[htbp]
    \sfig{#1.pdf}{0.45\columnwidth}
    \sfig{#2.pdf}{0.45\columnwidth}
   %  \end{center}
   \caption{#3} %{\small #2}}
    \label{fig:#1}
    \end{figure}
}

\newcommand{\rf}[1]{~\ref{fig:#1}}
 
\chapter*{Cosmic Visions Dark Energy: Science}
%\section{Dark Energy and CMB}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}\begin{boldmath}

\input authorlist.tex
%Conveners are also listed separately in authorlist.tex

\end{boldmath}\end{center}

\section*{Abstract}

Cosmic Surveys can probe fundamental physics.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\renewcommand*\thesection{\arabic{section}}
\section{Science} 

The spectacular success of the Standard Model of Cosmology is one of the most important scientific advances in human history. The universe began in a hot, dense state (the big bang), and expanded and cooled, initially going through a phase in which hot radiation was the dominant form of energy in the universe, leading to a clear prediction for the abundances of the light elements, stunningly verified through repeated observations. As the expansion continued, the energies of radiation and ordinary matter became comparable, and the hot radiation then streamed unhindered through the cosmos, to be detected 13 billion years later by our telescopes as the Cosmic Microwave Background (CMB). As matter became dominant, the inexorable force of gravity drew minor imperfections in its distribution into larger and larger aggregations, ultimately forming the complicated distribution of large-scale structure we see today.

This broad picture, based on gravity described through Einstein's theory of General Relativity (GR) and simple models of matter (relativistic and non-relativistic perfect fluids) provides a remarkable account of the behavior of the universe from around a minute after the big bang until relatively recent epochs. Like all good scientific stories, this explanation throws up an entirely new set of questions, the solutions to which demand an engagement with fundamental physics and promise to provide entirely new insights into that arena of enquiry. This is the goal of modern cosmology.

The flatness and homogeneity of today's universe, and the origin of the initial inhomogeneities that grew into galaxies cannot be explained within the confines of the standard cosmology, and require new physics active at extremely high energies. By far the best developed and most successful proposal is the idea that the early universe went through a brief period of accelerated expansion, smoothing out pre-existing inhomogeneities and curvature, while amplifying minute quantum fluctuations into small perturbations to seed large scale structure. This cosmic inflation is a general proposal that finds realizations in new high-energy particle physics models, making precise predictions for cosmological parameters, some of which have already been verified from observations of the CMB.

Details of the CMB, and a host of other cosmological and astrophysical observations, imply that the particle content of the standard model of particle physics is insufficient to account for how structure forms and behaves, and a new component of the cosmic energy budget is required, one that interacts at most weakly with itself and other particles. How this dark matter fits into a unified picture with regular matter is a question as pressing for particle physics as it is for cosmology. There exist a host of suggested candidates, with those that have garnered most attention arising from extensions of the standard model (SM) of particle physics developed to solve problems already existing in that model. Examples are Weakly Interacting Massive Particles (WIMPS), emerging from attempts to tackle the hierarchy problem of the SM, and Axions, resulting from a solution to the strong CP problem.

Perhaps most remarkably, it has become clear over the past 15 years, first through observations of type Ia supernovae (leading to the 2011 Nobel prize), and then supported by other measurements, that the very late time evolution of the universe is once again an accelerating state, with distant objects receding from each other at ever faster rates. As with inflation, this behavior presents a similar deep problem to fundamental physics, albeit at the completely opposite end of cosmic time. 

Cosmic acceleration suggests one of three logical explanations. One is that the cosmological constant (CC) is driving acceleration. This is a solution that would require the addition of a single new parameter to the CDM model, but that raises longstanding questions for fundamental theory. There currently exists no clear theoretical explanation of a CC of the required magnitude, except for the anthropic one, which requires a great deal of untested new physics. A second possibility is that there exists a new dynamical component to the cosmic energy budget -- dark energy -- driving physics similar to that needed for inflation, but at much lower energy densities, and without necessarily coming to an end. Such models come with their own theoretical baggage, but are a testable alternative to the CC. Finally, there is the possibility that regular and dark matter are the only sources of geometry, but that GR itself may be modified at very low energies/low densities/large scales -- modified gravity.

We have been forced to take each of the above problems of the standard cosmology seriously by repeated statistically significant anomalies in the increasingly precise cosmological data built up over the last few decades. In each case, it is possible to suggest a broad approach to the anomalies that contains the central physics required to explain the observations -- dark energy, dark matter, and inflation are examples of these. Building on these general paradigms, theorists have then been able to develop theoretically consistent frameworks, often, but not always built on the idea of weakly coupled quantum field theory coupled to gravity. Examples of these are quintessence and modified gravity models for cosmic acceleration; the lightest supersymmetric partner (LSP) WIMP candidate for dark matter; and the plethora of inflation models built from scalar field theories. One of the great strengths of these approaches is that theoretical consistency alone can place rather strong constraints on the types of models that one might consider viable, although, of course, one has to remain sufficiently open-minded when interpreting the data.

A challenge presented by these specific models is that the quantities that enter them are often not simply connected to the parameters that are measured by our experiments.  A paradigmatic example is given by late-time cosmic acceleration. Our first direct evidence for acceleration came from the lightcurves of type Ia supernovae. These allowed us to infer a precise Hubble diagram out to much further distances than before, with the resulting behavior of the cosmic scale factor indicating that the universe is not just expanding, but accelerating. GR coupled to normal perfect fluids such as baryons, dark matter and radiation cannot yield this behavior, and so we are led to the paradigm of dark energy. What this implies for fundamental physics now very much depends on how the behavior of spacetime is connected to the distribution of energy density in the Universe. If GR governs this, then either a cosmological constant, or some kind of dynamical dark energy is required. Alternatively, matter may remain quite mundane, and modified gravity may be responsible for what we are observing. 

Turning these ideas into concrete theoretical constructions requires sometimes highly complex and nontrivial studies. Many simple ideas can turn out to have fatal instabilities, while others may ultimately not admit self-consistent theoretical descriptions. The models that remain are often couched in the language of covariant Lagrangians for fundamental degrees of freedom - scalar fields, gravitons, etc.  While they may explain the required expansion history well enough, by construction, the success of attempts to further constrain them through cosmological observations depends on how well one can extract robust predictions for observables from these fundamental parameters. 

In the case of simple dark energy models, for example, the equation of state parameter, $w$, and its derivative, $w'$ (or parametric descriptions of this) have proven useful. Modified gravity models have forced us to look more deeply into structure formation, linking the fundamental models through linear perturbation theory to modifications to the growth functions and ultimately to features in the matter power spectrum. In a time when one cannot realistically expect any specific model to be completely correct, it is initially most important to be able to identify as many model-independent behaviors as possible in order to use the data as a discriminating tool against classes of ideas.

Similar arguments to this can be applied to dark matter and inflation, and the relationship between the initial observed anomalies all the way through to current and future observational targets is sketched in the table below. 

Neutrinos play a different role in cosmology. Their impact on the evolution of structure in the Universe is small but measurable. However, these measurements are directly tied to quantities, such as the neutrino masses and the existence of sterile neutrinos, that can also be directly probed in terrestrial experiments. The same cosmic surveys that will help us solve the mysteries of the dark sector and inflation will also provide complementary information about neutrinos, information that will either support the 3-neutrino, cosmological paradigm or upset it in ways that could reverberate through many sub-fields of physics.

%%%%%%%%%  ADDED BY MARK %%%%%%%%%%%%

\subsection{Theoretical Considerations}
Einstein gravity is remarkably robust. It represents the unique interacting theory of a Lorentz invariant massless helicity-2 particle. Therefore, essentially all new physics in the gravitational sector introduces new degrees of freedom, which are frequently Lorentz scalars. 
Perhaps the only exception to this is the cosmological constant itself, $\Lambda$.

The smallness of $\Lambda$ introduces two related, but essentially distinct, problems. The first is what is usually called the cosmological constant problem. This can be most succinctly phrased as the question: {\it why is the observed value of $\Lambda$ so small in Planck units?} Related to this is the question, usually referred to as the {\it coincidence problem}, which may be phrased as: {\it why is the energy density of this CC so close to the present matter density?} It is attempting to answer one or both of these questions that has led to various proposals for new physics.

One possible solution is that the cosmological constant is just small because a universe with a larger cosmological constant would not be able to support the formation of large-scale structures and the presence of life capable of asking why the cosmological constant is so small. Weinberg famously argued  that the cosmological constant should be within a few orders of magnitude of the upper bound which still allows cosmological structures to form, which is in very rough agreement with the value needed to explain observations. For this idea to make sense, it is necessary for the underlying laws of physics to allow for multiple realizations of the universe---in time, space, or both---with different values of the cosmological constant. Recently these {\it anthropic} ideas have gained new life, particularly within the context of the string theory landscape. However, even if all of the required ingredients can be established, it may nevertheless prove extremely difficult to show that the anthropic explanation is the correct one, and, of course, any experimental evidence that cosmic acceleration has a dynamical source would rule out such an answer immediately. Thus, it would be extremely premature to abandon the search for other theoretical explanations for cosmic acceleration.

\subsubsection{Dynamical dark energy}
Another intriguing possibility is that the ultimate value of the cosmological constant is zero, and that cosmic acceleration is due to the potential energy of a field, with some sort of mechanism to dynamically relax it to a small value. This notion naturally leads to models of {\it dark energy} which invoke a slowly-rolling cosmological scalar field to source accelerated expansion, akin to cosmological inflation. In such models it is difficult to see how to avoid fine tuning at the same level as just tuning the bare CC. Nevertheless, these dynamical dark energy models offer the simplest extension of $\Lambda$CDM and have been extensively studied. 

Such {\it quintessence} models have a rich phenomenology; one of the more interesting phenomena is that by suitably choosing the potential, the energy density in the field can be made to ``track'' the energy density in radiation/matter at early times and then grow to dominate the energy budget at late times.

Importantly, quintessence models must be very weakly coupled to matter, otherwise the scalar field will mediate a fifth force, in conflict with tests of gravity.  Absent some symmetry principle, setting the coupling to matter to be small is a fine tuning beyond that required to make the CC itself small (which is, itself, also required here), since if the coupling is set to zero classically, it will be generated through loops albeit with its resulting value suppressed by powers of $M_{\rm Pl}$. 


\subsubsection{Modified Gravity}

There are, in principle, a number of different ways to classify modified gravity theories. In fact, it is not completely clear how to perform such a classification distinct from dark energy theories in general, since in many cases they both involve new degrees of freedom. Common to most models though is the realization that any new gravitationally coupled degrees of freedom run the risk of being ruled out by local tests of gravity unless some new physics comes into play. Thus, we require mechanisms through which these new degrees of freedom are screened in the solar system, where most precision tests hold. 

One simple example of modified gravity that has received a lot of attention is so-called $f(R)$ gravity; in these models, the Ricci scalar in the Einstein--Hilbert action is replaced by an arbitrary function of the Ricci scalar. Models involving higher curvature invariants have been interesting to theorists since early investigations which showed in particular that a theory with quadratic curvature terms is renormalizable. In the context of inflation, Starobinsky wrote down a Lagrangian of the form ${\cal L} \sim R+R^2$ which was shown to be able to drive cosmic acceleration in the early universe. More recently, this idea has been adapted to explain the late-time acceleration of the universe, without invoking a cosmological scalar field. Since then, there have been numerous investigations involving models of this type. 

The action for this modification to Einstein gravity is of the form
%
\be
S = \frac{M^2_{\rm Pl}}{2}\int\rd^4x\sqrt{-g}\Big(R+f(R)\Big) + S_{\rm matter}[g_{\mu\nu}, \psi]~,
\label{fRaction}
\ee
%
where we have assumed that the matter fields, $\psi$, couple minimally to the metric $g_{\mu\nu}$, which has Ricci scalar $R$. In fact this theory is classically equivalent to a scalar-tensor theory. 

Such a modification to gravity is interesting because the additional scalar degree of freedom acts as another source in Einstein's equations, which can drive cosmic acceleration. Indeed, specializing to an FLRW background, by suitably choosing the functional form of $f(R)$, one can then reproduce any expansion history desired. in is worth noting, however, that the function $f(R)$ is not a completely free function, since there are various constraints on its form coming both from theoretical consistency and phenomenological viability. 

In particular, to avoid conflict with precision tests of gravity in the solar system, viable models of $f(R)$ gravity make use of the {\it chameleon mechanism}, through which the scalar field develops a density-dependent mass. Heuristically, the aim is to suitably choose the potential and non-minimal coupling to matter such that the mass coming from the effective potential is small in regions of low density and large in regions of high density, hiding the force from view. 

Another popular example of a modification to gravity is {\it massive gravity}.

Recall that Einstein's theory of gravity is the theory of a massless spin-2 particle, the graviton. The notion of giving this particle a mass and considering a theory of {\it massive gravity} has been intriguing to theorists since Fierz and Pauli's discovery of a unique ghost-free linear Lagrangian for a massive graviton, but until recently progress had come to a halt due to the powerful no-go theorem of Boulware and Deser~\cite{Boulware:1973my}, who had described the obstacles to finding a nonlinear completion of this theory. However, in the last few years, a loophole in these objections has been found, and an interacting theory of a massive graviton, free of the Boulware--Deser ghost, has emerged~\cite{deRham:2010ik,deRham:2010kj}. Interestingly,  massive gravity admits self-accelerating solutions in which the de Sitter Hubble factor is of order the mass of the graviton. Since having a light graviton is technically natural \cite{ArkaniHamed:2002sp,deRham:2012ew,deRham:2013qqa}, such a solution is of great interest in the late-time universe as a candidate explanation for cosmic acceleration. 



%
%
\noindent
{\bf Galileons in the decoupling limit:}\\\indent
The longitudinal polarization, $\phi$, of a massive graviton turns out to be described by a galileon theory in the decoupling limit 

\noindent
{\bf Self--accelerating solutions in the decoupling limit:}\\\indent
We now consider de Sitter solutions in massive gravity without external matter---self-accelerating solutions. As a first step, we search for these solutions in the decoupling limit, following~\cite{deRham:2010tw}.\footnote{See~\cite{deRham:2011by,Heisenberg:2014kea} for a discussion of the cosmology of a related covariantization of this theory.} 

In order for this to describe a de Sitter solution (with $H >0$) and for scalar and tensor perturbations about this solution to be stable, the parameters $a_2$ and $a_3$ must satisfy~\cite{deRham:2010tw, deRham:2012az}
\be
a_2 < 0~;~~~~~~~~~-\frac{2a_2^2}{3} < a_3 < -\frac{a^2_2}{2}~.
\ee
However, vector perturbations around the self-accelerating background appear to inevitably be either strongly-coupled or ghost-like~\cite{Koyama:2011wx, Tasinato:2012ze}.


\noindent
{\bf Cosmology away from the decoupling limit:}\\\indent
While we have focused on self-accelerating solutions in the decoupling limit, there have also been many studies of cosmological solutions in the full theory~\eqref{dRGTaction}. The situation is rather complicated. In~\cite{D'Amico:2011jj}, it was shown that the non-linear theory does not admit flat FLRW solutions. Nevertheless, there exist other cosmological solutions: open FLRW~\cite{Gumrukcuoglu:2011ew}, and cosmologies with anisotropies in the St\"uckelberg sector~\cite{Gumrukcuoglu:2012aa,Gratia:2012wt,Motohashi:2012jd,Kobayashi:2012fz,Maeda:2013bha}. However, perturbations about these solutions appear to be badly-behaved, both linearly~\cite{Gumrukcuoglu:2011zh,Koyama:2011wx,D'Amico:2012pi,Tasinato:2012ze,Fasiello:2012rw,Chiang:2012vh,Wyman:2012iw,Khosravi:2013axa} and nonlinearly~\cite{Kuhnel:2012gh,DeFelice:2012mx,DeFelice:2013awa}.


In order to remedy this situation and find acceptable cosmological solutions, many extensions of the dRGT theory have been proposed. One possibility is to let the background metric be dynamical, and consider a bi-metric theory~\cite{Hassan:2011zd,Baccetti:2012bk,Hassan:2012wr,Hassan:2012wt} (or even a multi-metric theory~\cite{Khosravi:2011zi,Hinterbichler:2012cn, Hassan:2012wt,Noller:2013yja}), leading to different cosmological solutions~\cite{Comelli:2011zm,Comelli:2011wq,vonStrauss:2011mq,Volkov:2011an,Volkov:2012cf,Volkov:2012zb,Comelli:2012db,Berg:2012kn,Akrami:2012vf,Volkov:2013roa,Tamanini:2013xia,Fasiello:2013woa,Akrami:2013ffa,DeFelice:2014nja,Solomon:2014dua}. Another possibility is to let the graviton mass itself be a field~\cite{Huang:2012pe, Hinterbichler:2013dv, Gumrukcuoglu:2013nza} or to couple in additional fields~\cite{Huang:2013mha,Kluson:2013yaa,Bamba:2013aca,Cai:2014upa,Wu:2014hva} (for instance galileon scalar fields~\cite{Gabadadze:2012tr,Andrews:2013uca,Goon:2014ywa}). One concrete proposal for adding new fields which has attracted some attention is so-called {\it quasi-dilaton} massive gravity, where the theory enjoys a scaling symmetry~\cite{D'Amico:2012zv}. Cosmologies of this theory and its extensions are considered in~\cite{D'Amico:2013kya, Gannouji:2013rwa,DeFelice:2013tsa,DeFelice:2013dua,Gabadadze:2014kaa}. A further enticing possibility is that a particular choice of the potential terms could lead to an extra gauge symmetry about de Sitter space, leading to a theory of {\it partially massless} gravity~\cite{Deser:2001pe,Deser:2001us}. This possibility has been explored~\cite{deRham:2012kf,Hassan:2012gz,Deser:2012qg,Hassan:2012rq,deRham:2013wv}, but it is not clear whether such a theory exists non-linearly~\cite{deRham:2013wv,Deser:2013uy,Joung:2014aba}.

Despite this flurry of activity, to date there does not seem to be an extension of dRGT which possesses a completely satisfactory self-accelerated solution. However, many of these extensions are interesting in their own right.

%%


In this section, we briefly discuss the status of massive gravity as applied to the real world. In this approach, the graviton mass is taken to be of the order of the present day Hubble parameter, m ? H0 ? 10?33 eV (for phenomenological bounds on the graviton mass see [27]). Although this is a very small parameter as compared to the Planck scale, such smallness is robust ? the mass parameter does not get renormalized by large quantum corrections [23, 28]; this is unlike the cosmological constant which does receive large renormalizations. Therefore, it is appealing to describe the observed cosmic acceleration as an effect due to a nonzero graviton mass.
Massive gravitons can produce a state with the stress-tensor mimicking dark energy (the so?called self-accelerated solutions [29?34]). Massive gravity dark energy is expected to have a slightly different predictions from those of CC based cosmology, and the differences may be tested observationally. These solutions produce dark energy with the equations of state identical to that of CC, but different fluctuations. Unfortunately, certain fluctuations about these solutions are problematic ? some of the physical 5 degrees of freedom have vanishing
kinetic terms, destabilizing the background [35]. Extensions of dRGT by additional scalars [31, 36] or bi and multi-gravity [9, 19], or further extensions [37, 38], also exhibit self- accelerated solutions. Recently, an extension by scalars has been proposed by De Felice and Mukohyama [39] and shown to have a self-accelerated solution with stable fluctuations ? a first example of this kind.

%%


\section{Screening with higher-derivative interactions: $\partial\phi; \partial^2\phi~\gsim~ \Lambda$}

In the effective Lagrangian, the only other types of terms that are generated beyond self couplings and couplings to matter are those terms involving derivatives of the new fields. When we write down our first field theories, we immediately encounter the simplest example of such a term as the kinetic term that is a quadratic term in derivatives of the field, and thus generates the evolution part of the resulting second order equations of motion. Indeed, even before thinking of field theories, it is the presence of the kinetic energy term in the Lagrangian for a point particle that gives rise to the acceleration part of $F=ma$. 




\subsection{Kinetic screening}
For simplicity, let us focus on scalar fields, generically written as $\phi$. Lagrangians with exotic kinetic terms, but involving only first derivatives of fields are often referred to as $P(X, \phi)$ models, with $X\equiv -\frac{1}{2}\partial_{\mu} \phi\partial^{\mu} \phi$, since the requirement that the Lagrangian be a Lorentz scalar means that the first derivatives must appear in this combination. 

Models of this type have been widely applied to cosmology. The simplest model of this type is a theory with a shift symmetry
\be
\phi(x)\longmapsto\phi(x)+c \ ,
\ee
where $c$ is a constant. For simplicity, we also imagine that the theory is invariant under the discrete symmetry $\phi \mapsto -\phi$

\subsection{The Vainshtein mechanism: galileons}
\label{galileonsection}

A related kinetic screening mechanism that has been of particular interest in recent years is the Vainshtein effect. This phenomenon is seen in some models arising from brane constructions in higher dimensions, and in limits of  theories of massive gravity~\cite{Vainshtein:1972sx,Deffayet:2001uk,Gruzinov:2001hp,Babichev:2009jt,Babichev:2010jd}. We will describe briefly a bit later how this effect is relevant to massive gravity. However, first, it is pedagogically simplest to describe the galileon theories, and how the Vainshtein effect manifests in them.

There are special classes of scalar field theories possessing higher derivative Lagrangians, but which nonetheless have second order equations of motion. It is now known that there are a large number of different examples of such theories, as we shall briefly discuss later, but the first to be discovered---and the canonical example---is the simple galileon theory. Galileons are higher-derivative field theories which are both invariant under the galilean shift symmetry
%
\be
\phi(x) \longmapsto \phi(x)+c+b_\mu x^\mu~,
\label{galileansymmetry}
\ee
%
and which have second order equations of motion. 

This symmetry initially appeared in the decoupling limit of the DGP (Dvali--Gabadadze--Porrati) brane-world, and was abstracted in~\cite{Nicolis:2008in} to a more general scalar field model. The restriction to terms which have second-order equations of motion is non-trivial---for example terms of the form $(\square\phi)^n$ are invariant under the symmetries, but have higher-order equations of motion.\footnote{As reviewed in Appendix~\ref{OstrogradskyApp}, higher-order equations of motion can lead to Ostrogradsky-type instabilities and the propagation of additional ghost-like degrees of freedom.}



Remarkably, there are a finite number of terms ($d+1$ in $d$-dimensions) that satisfy these combined requirements of invariance under \eqref{galileansymmetry} and second order equations of motion. 
Also interesting for our purposes is that each galileon term in the Lagrangian is not strictly invariant under the symmetries \eqref{galileansymmetry}, but rather  shifts by a total derivative, leaving the action invariant. It was shown in \cite{Goon:2012dy} that this is a natural consequence of the fact that the galileons are Wess--Zumino terms for spontaneously broken space-time symmetries, as we will discuss briefly.

Although galileons originally arose in brane-world modifications of gravity, they have appeared in other well-behaved modifications of gravity, for instance massive gravity \cite{deRham:2010ik,deRham:2010kj}. Further, models termed ``galileons" in the literature has grown far beyond theories invariant under the symmetry~\eqref{galileansymmetry}; indeed, galileon has become nearly synonymous with well-behaved derivatively-coupled theory.


The galileons have been used to address cosmic acceleration \cite{Chow:2009fm,Silva:2009km,Kobayashi:2009wr,DeFelice:2010as,DeFelice:2010gb,DeFelice:2010pv,Gannouji:2010au,Ali:2010gr,Mota:2010bs,Barreira:2012kk} and the origin of density perturbations in the early universe through inflation \cite{Anisimov:2005ne,Kobayashi:2010cm,Burrage:2010cu,Creminelli:2010qf,Kamada:2010qe,DeFelice:2010nf,Kobayashi:2010wa,DeFelice:2011zh,Kobayashi:2011pc,RenauxPetel:2011uk,Fasiello:2013dla} and inflationary alternatives \cite{Creminelli:2010ba,Hinterbichler:2011qk,LevasseurPerreault:2011mw,Wang:2012bq,Liu:2011ns,Hinterbichler:2012mv,Hinterbichler:2012fr,Hinterbichler:2012yn,Creminelli:2012my}. 



\subsubsection{Degravitation}


Massive gravity also allows us to view the cosmological constant problem in a different light. Rather than asking: {\it why is the observed cosmological constant so small?} we are able to ask the slightly different: {\it why does the cosmological constant not gravitate very strongly?}~\cite{Dvali:2002pe,ArkaniHamed:2002fu,Dvali:2007kt} This is an interesting viewpoint; up to now we have been fighting $\Lambda$, trying to make its value small, but this allows us to take seriously the notion that the large cosmological constant generated via matter loops is physical, and that it does not strongly curve space-time. This phenomenon of {\it degravitation} is intimately tied to massive gravity: as we will see below, any theory that exhibits degravitation must reduce, to a theory of massive/resonance gravity at the linearized level~\cite{Dvali:2007kt}. Moreover, degravitation admits a nice analogy with electromagnetism---it is the gravitational analogue of the screening of charges in a superconductor (Meissner effect)~\cite{Dvali:2007kt}.


\subsection{Horndeski theory}

A general question that we might ask is {\it what is the most general Lagrangian which couples a scalar field to gravity non-minimally, and which has second-order equations of motion}? This question precisely was asked and answered in~\cite{Deffayet:2009mn}, inspired exactly by this interest in covariantizing the galileon theory, and the resulting theory was referred to as that of {\it generalized galileons}.
It turns out that the answer to this question was known much earlier, but had gone mostly overlooked in the literature (but was resurrected in~\cite{Charmousis:2011bf}). In 1974, Horndeski~\cite{Horndeski:1974wa} wrote down the most general scalar-tensor Lagrangian which has second order equations of motion. It was pointed out in~\cite{Kobayashi:2011nu} that the generalized galileons and Horndeski's theory are equivalent (see~\cite{Kobayashi:2011nu} for a dictionary translating between the two languages). The Horndeski theory involves 4 free functions of the field and its kinetic term, and can be written as (in the notation of~\cite{Kobayashi:2011nu})

This theory has been constructed to have second-order equations of motion, but beyond that there are no symmetry properties which restrict the arbitrary functions. However, it is possible to place restrictions on these terms from their phenomenology. A basic phenomenological requirement is that the fifth force mediated by $\phi$ be screened from solar system tests~\cite{DeFelice:2011th,Koyama:2013paa}. 

Note that this theory evades Weinberg's no-go theorem about self tuning (reviewed in Appendix~\ref{Weinbergnogo}) by allowing for the profile of the field $\phi$ to be time-dependent. However, in order for such a theory to be observationally viable, it must employ the Vainshtein mechanism within the solar system to evade fifth force constrains, and recently it has been argued that the need for solar system screening and weak-coupling constrain the cosmological impact of the Fab Four~\cite{Kaloper:2014xya}.

Horndeski's theory has been extensively studied, for overviews see~\cite{Deffayet:2013lga,Charmousis:2014mia}. It has been used to construct general theories of inflation~\cite{Kobayashi:2011nu, Gao:2011vs,Gao:2011qe,Burrage:2011hd,Ribeiro:2011ax,DeFelice:2011uc,RenauxPetel:2011sb,DeFelice:2013ar} and cosmic acceleration~\cite{DeFelice:2011hq,DeFelice:2011bh,Leon:2012mt,Bloomfield:2011np,Bloomfield:2012ff,Bloomfield:2013efa,Mueller:2012kb,Tsujikawa:2014mba}. Additionally black holes have been studied in this theory in~\cite{Charmousis:2012dw, Babichev:2013cya,Anabalon:2013oea,Sotiriou:2013qea,Kobayashi:2012kh,Kobayashi:2014wsa,Charmousis:2014zaa}, and it has been generalized to describe multiple fields non-minimmally coupled to gravity~\cite{Padilla:2012dx, Sivanesan:2013tba,Padilla:2013jza}.

Finally, note that expanding Horndeski's theory about a cosmological FLRW solution neatly leads to a type of EFT of dark energy, similar to the theories discussed in~\cite{Park:2010cw,Creminelli:2008wc,Bloomfield:2012ff,Gubitosi:2012hu,Gleyzes:2013ooa,Piazza:2013coa,Frusciante:2013zop,Bloomfield:2013efa,Gergely:2014rna}. Additionally, the fact that expanding the general Horndeski theory about a cosmological background in the quasi-static regime requires two functions of time and scale to describe perturbations connects to the parameterized post-Friedmann approach to modified gravity, which we discuss briefly in Sections~\ref{quasistaticsec} and~\ref{section:PCA}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Surveying more objects at higher redshift}

In particle physics, the new physics discovery potential of new experiments depends, broadly speaking, on two factors; increasing the energy of collisions and increasing the luminosity of accelerators. As the LHC increases its energy, it will access new states not accessible at lower energy. As it increases its luminosity, LHC will produce, for example, many more Higgs particles, and their various decay modes can be measured more and more accurately. Furthermore, increased luminosity means that even very rare events in, for example, the decay of lighter particles, may be discovered at the statistically significant level. If the partial widths to any of these channels, for any such decays, disagree with those predicted by the Standard Model, we will have evidence for new physics. The key though is to generate enough interactions, or to produce enough Higgs particles, to enable these careful statistical determinations.

An analogous pair of considerations are relevant to the problem of extracting new physics from cosmic surveys. In this case, the analog of the unexplored frontier of higher energy is higher redshift and the analog of luminosity is the number of objects tracing the underlying density field. DESI and LSST carry so much promise because they will both explore the universe out to higher redshift and detect many more objects than previous surveys such as DES and SDSS. These increases in both the "energy" and "luminosity" of our next generation of surveys provide complementary ways to increase their discovery potential.

The benefits of increasing the number of objects we measure are simplest to understand when applied to measuring the redshift-distance relation using the Baryonic Acoustic Oscillation feature. As indicated in Fig.~\rf{currentdistance}, DESI will obtain percent level measurements on distances out to redshift $z=3$, and this will open up possibilities of discovery especially when it comes to understanding the physics driving the current epoch of acceleration. The right panel of Fig.~\rf{currentdistance} shows that we can hope to tighten the constraints on this relation at high redshifts by a factor of ten by measuring even more objects in the future.

\Sfigtwo{currentdistance}{distances}{Projected errors from an all-sky survey on cosmic distances using the Baryon Acoustic Oscillation feature. Left panel shows what is expected with DESI; right shows the potential even after DESI successfully concludes. Especially at high redshift, the measurements can be made more precise by up to a factor of 10. (From the Snowmass Distance document.)}

It is not just distance measures that can be measured more accurately; higher redshift and more tracers of the mass density enable us to measure {\it inhomogeneities} more accurately. Fig.~\rf{power} shows why this is so important. Fundamental quantities like the dark energy equation of state, the sum of the neutrino masses, or the shape of the primordial spectrum generated during inflation leave their imprint on these inhomogeneities. The {\it power spectrum} quantifies the level of inhomogeneity as a function of scale and redshift and therefore encodes the impact of these fundamental quantities. As surveys explore higher redshifts, they can explore the power spectrum at those epochs and -- as the right panel of Fig.~\rf{power} shows -- become sensitive to features in the power spectrum that vary with time. This corresponds to finding new modes at higher energies in a collider.

Akin to increasing the luminosity, the more tracers that are surveyed at a given redshift, the more accurately will this power spectrum be measured. As the left panel of Fig.~\rf{power} shows, it is important to accurately measure the power spectrum as a function of scale, so the higher accuracy makes it more likely that we will find find new physics. In other words, small effects at lower redshifts are analogous to rare events or decays at lower energies in particle physics. Only by increasing the "luminosity" - the number of objects we can measure - can we reduce the error bars to a level where these small effects poke up above the statistical noise.

\Sfigtwo{power}{growth}{Changes in the power spectrum due to: {\it Dark Energy} equation state $w=-.95$, {\it Inflation} spectrum with running $dn/d\ln(k)=0.01$, and {\it Neutrino} masses summing to 60 meV. Left panel shows changes as a function of scale; right panel as a function of time or redshift.}

By detecting more objects at high redshifts then, we can obtain better precision measures of the inhomogeneities. Fig.~\rf{dpower} shows these projected improvements as a function of the number of objects detected. While DESI will do almost as well as possible at $z=1$, there will remain an enormous amount of information lurking at higher redshifts. To extract all of this information and learn as much as possible about fundamental physics, future surveys will have to measure more objects at redshift $z>1$.

\Sfig{dpower}{Fractional error in $P(k=0.2)$ for various redshifts as a function of the number of objects surveyed. The dots are projections for DESI: at $z=1$ DESI will be within a factor of 3 of the ultimate error, but at higher redshift, there is at least of factor of ten more information to be mined by future surveys.}

Graph with constraints on each of $\sim10$ parameters ($w,w_a,\sum m_\nu,n',f_{NL}, D(z),\ldots$). For each one, show: Current,  projected range for DESI and LSST [w/ and w/o enhancements], and using all Fourier modes

\section{Enhancing DESI and LSST}

\begin{itemize}
\item {\bf Theory} 
\item {\bf Photometric redshift calibration} 
%\item Ideas that seem less compelling are Spherex and MKIDS
\item {\bf Spectroscopy for LSST-discovered Supernovae and Strong Lenses}
\item {\bf Cross-Correlation with other experiments} For bias uncertainties in DESI, cross-correlation with lensing maps will help. Stress importance of standardizing data formatting and exchange with CMB experiments as well as WFIRST, Euclid. Co-siting CMB-S4 with LSST will help with bias, multiplicative shear calibration, cluster masses, and even photometric redshift calibration.
\item {\bf Novel Probes}
\item Small scale power spectrum from microlensing with ALMA constrains dark matter mass (not really an enhancement of DESI, LSST but small-ish scale thing that we might raise)
\item {\bf Kinematic Weak Lensing}
\item {\bf Cluster Velocity Dispersions}
\item {\bf Simulations}

Simulation and modeling efforts play a central role in modern cosmological
surveys. Broadly speaking, simulations serve three main purposes: (i)
solving the inverse problem, meaning inferring cosmological information
from the data, (ii) generating synthetic sky catalogs at different wavebands for pipeline and algorithm validation, and (iii) end-to-end simulations of the full survey or
parts of it.

The first category includes the exploration of the impact of fundamental physics -- e.g., massive neutrinos,
dynamical dark energy, modified gravity models, dark matter
self-interaction, and features in the primordial power spectrum
-- on observables, . In ongoing and up-coming
surveys we hope to extract new cosmological information from nonlinear
scales, therefore simulations will be essential to provide the necessary
predictions over a wide range of cosmological models and scales. Simulations are
also crucial to investigate astrophysical systematics in detail, such
as the effect of baryonic physics on the power spectrum or the mass
function. Finally, as part of solving the inverse problem, estimates of the
covariance matrix rely heavily on simulations. Currently, brute-force
methods for generating covariances from simulations are
computationally too costly and new approaches for obtaining
covariances are being actively investigated.

Synthetic sky catalogs serve several purposes. They allow for detailed validation
of analysis pipelines and algorithms. The important fact here is that
the {\it truth} is known and the catalogs can be used to carry out tests in 
controlled ways. They therefore also can form the basis for data challenges
to prepare the analysis teams for real data and understand if their analysis software is up to the task of extracting the subtle signals under investigation. In addition, they can be used to mimic realistic data rates from the surveys to ensure scaling of the analysis codes. 

End-to-end simulations of the full survey have started to become
possible; for example, LSST will attempt to have a full
modeling pipeline starting from simulated synthetic skies (as described above) to modeling
of the atmosphere and the telescope optics to the detectors in order
to generate images as close to the real observations as
possible. Other surveys have also carried out simulations of parts of
this pipeline.  These simulations are very important to understand
systematics effects in the observations themselves that can be induced
due to the observational hardware, calibration issues, or data
analysis pipeline shortcomings. Detailed simulations allow us to
investigate those possible systematics and their effects on the data
and cosmological constraints and to mitigate them eventually.

Given this overview, what are the challenges facing simulations?

First, the accuracy requirements for our predictions are daunting,
given the forecasts for the measurement errors expected from LSST and DESI. A concrete example is the inclusion of massive neutrinos
within the simulations. While many approximate methods have been
developed to make neutrino simulations computationally feasible, a
full understanding of the errors due to the approximations has not
been carefully developed on all scales. Another major challenge with
regard to accuracy is the modeling of different types of galaxies at
different depths on top of the gravity-only large scale structure
backbone information. Again, a range of methods has been developed for this task
but so far, none of them is fully satisfactory in reproducing all of the
observational data (creating a detailed observational
validation set that can be used for this task is another major
challenge). Overcoming these obstacles will be very important if we attempt to extract
information from small scales to constrain cosmology.

Modeling of astrophysical effects via hydrodynamical simulations is
another major challenge. Currently, results from different simulations
vary considerably on scales smaller than 1 Mpc. While mitigation strategies
are being developed, we might ultimately lose some information on
small scales if we cannot improve our modeling and simulation
approaches. In addition, some astrophysical effects can mimic
cosmological physics. We have to guard against drawing incorrect
conclusions due to a lack of understanding of these effects.

A different (and very exciting) challenge will arrive if evidence emerges for physics beyond the cosmological constant. Currently, we
have no large, very detailed simulations for modified gravity (MG)
theories for several reasons. One reason is that it is not fully clear
how to best explore different MG theories in a systematic
way. Secondly, our current approaches are computationally very
expensive. But given the fact that most information again is hidden on
small scales, a simulation approach is essential.

Ongoing and upcoming surveys target a large variety of
cosmological probes in order to explore cosmological constraints
in multiple ways. From the modeling and simulation aspect, this
however poses another major challenge. Each probe requires specific
modeling approaches on top of the raw simulation outputs and different
levels of detail.

In order to be fully prepared for the upcoming surveys we need a concerted effort for modeling and simulations similar to the effort developed for high-energy physics experiments.

%To summarize, simulations play an important role in many aspects of
%ongoing and upcoming surveys, including modeling and understanding of
%fundamental physics, astrophysical effects, systematic effects,
%testing of pipelines and to provide data challenges for the
%surveys. They will be crucial in case we discover new physics to guard
%us against incorrect conclusions. 
\end{itemize}

\section{Next Big Cosmic Survey}


\subsection{Spectroscopy}

\href{https://indico.bnl.gov/getFile.py/access?contribId=8\&resId=0\&materialId=slides\&confId=1406}{Billion Object Apparatus}



\subsection{Hydrogen and Carbon Surveys}

\href{https://indico.bnl.gov/getFile.py/access?contribId=4\&resId=0\&materialId=slides\&confId=1406}{21 cm}

%%
%% Populate the .bib file with entries from SPIRES Bibtex (preferred)
%% or ADS Bibtex (if no SPIRES entry).
%%  SPIRES will also supply the CITATION line information; please include it.
%%

%\end{document}


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

